Characterizing the Landscape of COVID-19 Themed Cyberattacks and Defenses

COVID-19 (Coronavirus) hit the global society and economy with a big surprise. In particular, work-from-home has become a new norm for employees. Despite the fact that COVID-19 can equally attack innocent people and cybercriminals, it is ironic to see surges in cyberattacks leveraging COVID-19 as a theme, dubbed COVID-19 themed cyberattacks or COVID-19 attacks for short, which represent a new phenomenon that has yet to be systematically understood. In this paper, we make the first step towards fully characterizing the landscape of these attacks, including their sophistication via the Cyber Kill Chain model. We also explore the solution space of defenses against these attacks.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> case-study.tex <==

%{\color{red}We have discussed a lot of attacks in previous sections. The case study can defense a subset of the attacks. We should mention the scope.}
%\subsection{Scope}
In this section we present a case study on detecting COVID-19 themed malicious websites.

Figure \ref{fig:detectionFramework} highlights the detection framework, which is based on multiple state-of-the-art machine learning models depicted as $C_1, C_2, C_3, \dots C_K$.\footnote{I do not think it's important to stress ensemble learning, because it is just one case of the models; moreover, random forest is already an ensemble learning} which can be decomposed into the following modules: data processing, classifier training, and classifier testing.
%\footnote{re-draw the picture to reflect these three modules, {\color{orange}Done}}

\begin{figure}[!htbp]
\centering
\includegraphics[width=1.05\linewidth]{figures/DetectionFramework.pdf}
\caption{Framework for detecting COVID-19 themed malicious websites }
\label{fig:detectionFramework}
\end{figure}



%domains that are involved specially in phishing, scamming, and social engineering attacks. In this section we discuss about the relevant dataset, pre-processing, feature extraction, insights from the data, the framework architecture, evaluation criteria, and experiment results. This case study is a pilot project to show how we can effectively and proactive defend against the COVID-19 themed malicious websites.
%\subsection{Problem Statement} Given a set of COVID-19 themed websites mixed with other benign websites, can we identify the impactful features (lexical, host-based, WHOIS-based, content-based, or keyword-based) for classifying websites which can accurately identify the `malicious' ones from the `benign' ones? are intentionally created by the attackers to which wage various COVID-19 themed cyberattacks. To illustrate, if we are given a set of COVID-19 themed websites $W_{covid}$, can we accurately classify the malicious COVID-19 themed websites, $W_{malicious}$, from the set of benign websites, $W_{benign}$? Here, $W_{covid} = W_{malicious} \cup W_{benign}$. 
% where $W_{benign}$ presents the COVID-19 themed benign websites.  

%As most of the IT enterprises are moving to WFH model it is important to detect these malicious websites and minimize the risks. 

\subsection{Data Collection and Pre-Processing}
%\subsubsection{Dataset Selection}
%For this case study, we first analyze the existing data sources for COVID-19 themed websites. 
\subsubsection{Initial Data Collection}
Our dataset consists of COVID-19 themed malicious and reputed benign websites. The malicious websites are obtained by taking the union of two sets of websites respectively published by the following two sources between 2/1/2020 and 5/15/2020:
%(while removing duplicates): 
(i) CheckPhish \cite{COVID19_data_checkphish}, which covers websites with 
%current or potential future 
scamming attack schemes related to COVID-19;
%. They publish the scam websites on a daily basis starting from February 1, 2020, that are related to COVID-19 pandemic. They also publish a worldwide geographical map of these scamming attacks in their dashboard to show the attack trends in different geo-locations.  
%{\color{red}...better add some description similar to DomainTools ...}
%From this source, we collected `malicious' labeled websites between 2/1/2020 and 5/15/2020. However, date information is not used for the detection framework presented in the case study. 
(ii) DomainTools \cite{COVID19_data_DT}, which provides COVID-19 related high-risk websites 
%with risk scores 70 or above on a scale of 100. The websites are mainly 
covering malware, phishing, and spamming attacks.
%From this source, we collected these high risk websites\footnote{did you set the threshold of high? if yes, what is the threshold score and explain why; if no, delete this sentence; {\color{orange}No the publisher of the dataset set this threshold and reported it while publishing}} and labeled them as malicious.
%\footnote{take note on idea for another research paper: reverse engineering the formula that were used by this vendor to rank websites ... then we can investigate its strength and weakness}
%between 1/1/2020 and 5/15/2020. However, date information is not used for the detection framework presented in this case study.
For obtaining benign websites, we use the top {\color{red}100,000} websites from Cisco's Umbrella 1 million websites dataset, which is a source of reputable websites. In total, we collected {\color{red}226,000} malicious websites and {\color{red}100,000} benign websites.\footnote{{\color{orange}need to revise these numbers after revisiting the experiments}}


%and add them to our `benign' labeled data to resolve the data imbalance problem \cite{kotsiantis2006handling}.
\ignore{
\item {\color{red}Malware Patrol \cite{COVID19_data_malPatrol}:\footnote{actually, we probably do not need this dataset, because 96\% of it are already covered by the two datasets mentioned above, {\color{orange}yes we can remove this dataset, will not make much of a difference in the result and also no need to make assumptions that malware patrol 4\% data is safe}} (data dated from March 1, 2020, to May 15, 2020), where the company shares the COVID-19 related website data `as-is' without any assumptions on suspiciousness. 
DomainTools and CheckPhish have the larger sets of COVID-19 malicious websites with more coverage, so it is safe\footnote{no, it's not safe to make this assumption; instead, we should use this dataset as a part of the test set; for benign website, we'd use more reputable website} to assume the remaining websites in Malware Patrol's data that are not reported in either of the CheckPhish and DomainTools as `benign' COVID-19 themed websites.
While merging Malware Patrol's COVID-19 new domain dataset with our `malicious' labeled set we only merged the new websites that are not reported in either of the two `malicious' labeled data sources as our `benign' label websites. However, our merged list has produced around 96\% `malicious' labeled data points and only 4\% `benign' labeled data points which bring the imbalance dataset problem for training the machine learning classifiers.}\footnote{rewrite the entire paragraph: by treating the 4\% as test dataset; we cannot use a dataset of which 96\% are malicious and then 4\% as benign} 
}

%Multiple sources have been collecting and publishing daily COVID-19 feeds \cite{COVID19_data_malPatrol, COVID19_data_DT, COVID19_data_checkphish, COVID19_data_phishlab} or publishing some historical real-world data \cite{COVID19_data_spycloud, COVID19_data_sophos}. %To generate our set, we aggregate COVID-19 themed website data from three sources to get our training and testing data with ground-truth labels. 
%Thus, connecting the above dataset gives our model more coverage and makes it more robust against detecting malicious COVID-19 themed website. 
%The Malware Patrol's data is published `as-is' with no assumption of malicious or benign labels daily from March 1, 2020, till present.
%On the other hand, DomainTools data \cite{COVID19_data_DT} is publishing only high-risk COVID-19 websites (suspicious scores 70 and above out of 100) with dates, which we labeled as malicious in our dataset. Next, CheckPhish Scam Tracker \cite{COVID19_data_checkphish} also publishes COVID-19 related malicious websites with labels (such as phishing, scamming, spam, and suspicious) with date labels from January 2020. 

%\subsubsection{Pre-process Data}
%The CheckPhish COVID-19 scam feeds are labeled as `scam' and `suspicious' while the DomainTools %153,216 unique 
%COVID-19 threat list has the high-risk websites with their risk-scores. We combine these two datasets and remove the duplicate websites to build our `malicious' labeled dataset. 
%along with the uncertainty that    website. Moreover, we have also collected top 100,000 benign websites from Cisco Umbrella 1-million dataset \cite{cisco_umbrella_dataset} to resolve the imbalance dataset problem .  

%where a new unseen portion of. Next, we merge CheckPhish, and DomainTools labeled datasets and remove the date, and duplicate websites used for the ground truth labeled data. Then, we merge this labeled data to Malware patrol's unlabeled data (removing duplicate websites), which yields 236,606 unique websites with 226,838 `malicious' and 9,768 `benign' labeled COVID-19 themed websites. Next, we further refined the dataset and removed websites with no WHOIS registration information. We assumed those websites were possibly detected by publicly available blacklists and might have been removed already. 


%The benign labeled data contains 47,992 top Cisco websites 
%Finally, for this classification problem the `malicious' labeled dataset contains 50K COVID-19 themed malicious websites (compiled from CheckPhish and DomainTools) randomly chosen from an available 154,965 websites and the `benign' labeled dataset contains 50K websites randomly chosen from an available 53K benign websites (compiled from Malware Patrol and Cisco Umbrella top 100K websites). 

%We generate the pre-processed COVID-themed \textit{`malicious dataset'} ($W_{malicious}$) containing $154,665$ unique websites by combining CheckPhish and DomainTools data %and removed the website that are created before 1 December, 2019. 
%Next, we  joined pre-processed COVID-themed benign data of around $10K$ unique websites with Cisco Umbrella $100K$ benign websites to generate our \textit{`benign dataset'} ($W_{benign}$) of about $110K$ websites. 

%We pre-process the features for top 100,000 websites to remove data points those do not have any valid \textit{WHOIS registration date} extracted from the server. We observe that around 52K top websites did not have a valid registration date retrieved thus we remove those data. In our final dataset we have 108K websites with 58K being malicious' ($W_{malicious}$) and 50K being 'benign' websites ($W_{benign}$). Further, among our benign data we have 47,974 websites from Cisco whereas the remaining 2,019 websites are COVID-19 themed benign websites. Thus, making size of the COVID-themed websites, $|W_{covid}|=60,000$. The brief of the data pre-processing steps are shown in Figure \ref{fig:dataprocessing}. 
%Moreover, We also capture unlabeled and labeled new COVID-19 %websites data from Malware patrol, DomainTools, and CheckPhish after %May 15, 2020 to evaluate the effectiveness of our model for predicting %new COVID-19 related unknown (zero-day) malicious websites.

\ignore{
\begin{figure}[!htbp]
\centering
\includegraphics[width=1.03\linewidth]{figures/data_preprocessing.pdf}
\caption{Data prepossessing steps {\color{red}[Proccesing steps changes, will update this figure]}}
\label{fig:dataprocessing}
\end{figure}

\begin{table} [!htbp]
  \caption{Snapshot of the Selected Pre-processed Datasets}
  \label{tab:datasetDescription}
  \begin{tabular}{|c|c|c|c|c|}
    \toprule
    Data  & Date & Coverage & \# of Unique \\
     &  &  &  Websites\\
    \midrule
%    CheckPhish & 02/01/20 to & scam \&  & 150,216 \\
%            & 05/15/20 &  suspicious &  (duplicates?)\\
%    \midrule
%    DomainTools & 01/01/20 to & phish, spam,  & 154,965\\
%        & 05/15/20 & malware &  (duplicates?)\\
%    \midrule
%    Malware Patrol & 03/01/20 to & assumed benign & 5,009\\
%            & 05/15/20 &  & \\
%    \midrule
%    Pre-proccessed & 06/12/20 & benign & 47,992\\
%    Cisco Umbrella  & & & \\
%    \midrule
    Pre-processed & 01/01/2020 to & scam, spam, & 154,674\\
    COVID-19 themed & 05/15/20 & phish, malware & \\
    `malicious' data & & & \\
    \midrule
    Pre-processed & N/A & benign & 47,992\\
    `benign' data &  &  & \\
    \midrule
    \bottomrule
  \end{tabular}
\end{table}
}



\subsubsection{Feature Definition and Extraction} \label{sec:features}

%We extract various features for malicious website detection and analyze which of these features' combinations fitting well for our COVID-19 themed malicious website detection framework. 
In order to detect COVID-19 themed malicious websites, we propose defining features related to websites' lexical, statistical, WHOIS-based, domain-based, and keyword-based features.
%\subsubsection{Feature Definition}
%\subsubsection{WHOIS-based features}
\begin{itemize}
\item WHOIS registration lifetime ($F1$): This is the number of days that has passed since a website' WHOIS registration date, with respect to the date when this feature's value is extracted  (e.g., 5/16/2020 in our particular dataset).
%as of 16 May, 2020 when we make the query to the WHOIS service.

\item Remaining WHOIS expiration lifetime ($F2$): This is the number of remaining days before a website's WHOIS registration expires, with respect to the date when this feature's value is extracted (e.g., 5/16/2020 in our particular dataset).  

\item Number of days since WHOIS' last update ($F3$): This is the number of days elapsed since the website is last updated %{\color{red}...update on what? information about a website ... or something else ... be precise rather than ask the reader/reviewer to guess ...}, 
with respect to the date when this feature's value is extracted (e.g., 5/16/2020 in our particular dataset).

%\subsubsection{Lexical features}
\item Number of dots in domain name ($F4$): This is the number of dots (character `.') in the domain name. For example, a website {\tt any.com} has 1 dot.
%in {\color{orange }it hence the dot count is 2.}  %{\color{red}but there is one `.' character in the domain name `any.website' and thus has a dot count of 1, while noting that {\tt .com} is called the Top-Level Domain (TLD) for this website.}
%\footnote{revise: do not call that domain name; when we say domain name, we say it as a whole; of which, TLD is just one component; revise this and the code for data processing etc; \color{orange} okay, I will address it in the re-experiments} 

\ignore{
\begin{table} [t]
  \caption{List of `generic' and `bad' registrars}
  \label{tab:registrarList}
  \begin{tabular}{ll}
    \toprule
    Generic registrars & Akamai, Alibaba, Godaddy, Google \\  
    & domains, Domain.com, Namecheap,  \\ 
    & name.com, CSC Corporate Domains, \\
    & markmonitor, 1\&1, dreamhost, hostinger, \\ & registrarsafe, network solutions, \\
    &  ovh, register.com \\
    \midrule
    Abused registrars\cite{bad_registrar_list} &  namesilo, dynadot, gmo, r01-ru, nawang\\
    & eranet, net-chinese, zhengzhou, shinjiru\\
    %& '阿里巴巴云计算（北京）有限公司'\\
    

    \bottomrule
  \end{tabular}
\end{table}
}


\item Domain entropy ($F5$): This is the Shannon entropy \cite{shannon_entropy} of the domain name, which is computed based on the frequency of symbols in the domain name.

\item Domain length ($F6$): This is the length of a domain name, including dots and TLDs. For example, the length of domain {\tt any.com} is 7.
%{\color{red}domain {\tt any.website} for a website {\tt any.website.com} is 11.}\footnote{same problem as mentioned above; revise}

\item Domain digits count ($F7$): This is the number of digits (i.e., 0 to 9) in a domain name. 
\item Domain hyphen count ($F8$): This is the number of hyphens (`-') in a domain name. 

\item Domain vowel count ($F9$): This is the total number of vowels in a domain name.

\item Domain digits percentage ($F10$): This is the percentage of digits (0-9) in a domain name, namely $F7/F6$. We include $F6$ and $F7$ because they may contain more information that is not captured by $F10$.
%\footnote{we already know this feature is derived from the other two, do we have to consider this one? {\color{orange} Actually this one is better than those two, we I defined it separately but while calculating the Pearson correlation definitely this three will be strongly correlated and I will delete the previous two F6/F7; if you are olay we can remove F6, F7 and only keep F10 by adding the description in F10}}
%It is the ratio of the `digit count' and  `domain length'.

\item Domain unique alpha-numeric characters count ($F11$): This is the total number of unique alpha and numeric characters (i.e., a-z, A-Z, 0-9) in a domain name.

\ignore{
\begin{table} [ht]
  \caption{List of `generic' and `abused' TLDs}
  \label{tab:tldList}
  \begin{tabular}{ll}
    \toprule
    Generic TLDs & .com, .net, .org, .xyz, .ru, .uk, .fr, .it, .info \\
    \midrule
    Abused TLDs & .live, .buzz, .gq, .tk, .fit, .cf, .ml, .wang, .top, .rest, 
    \\& .work\\
    \bottomrule
  \end{tabular}
\end{table}
}

\item Top-Level Domain (TLD) features ($F12$-$F14$): There have been studies on characterizing the 
%We create a list of {\em generic}  and {\em abused} TLDs based on the popularity among the reputed websites and the 
{\em badness} of TLDs \cite{bad_TLDs_2020,bad_TLDs_all_time}.
%, which publish the top ten most abused TLDs till date and other TLDs can be queried to extract the associated {\em badness} index. 
{\color{red}From this source, we obtain: (i) a list of {\em generic} TLDs (i.e., .com, .net, .org, .xyz, .ru, .uk, .fr, .it, and .info), each of which has been hosting no more than 5\% malicious domains; and (ii) a list of {\em abused} TLDs (i.e., .live, .buzz, .gq, .tk, .fit, .cf, .ml, .wang, .top, .rest, and .work), each of which contains least 30\% abused domains.
%where TLDs hosting domains of which around 30\% to over 50\% are bad domains.and ??? {\em abused} TLDs.
Correspondingly, we define three binary features:
%{\em generic}, {\em unknown}, and {\em abused} TLDs. into two classes: {\em unabused} vs. {\em abused}. 
$F12$ indicates a website is {\em benign} or not; $F13$ indicates a website is {\em abused} or not; $F14$ indicates if a website is neither benign nor abused.}\footnote{why not simply using the abusedness as a domain's feature? why you have to define three features?} 
%{\em unknown} or not`1' if the input website is in the {\em abused} TLDs list, and `0' if it does not appear on the {\em abused} list. Our list of generic TLDs contains .com, .net, .org, .xyz, .ru, .uk, .fr, .it, and .info where none of these TLDs hosting bad domains exceeding than 5\% of their active domains. On the other hand, the list of abused TLDs contains .live, .buzz, .gq, .tk, .fit, .cf, .ml, .wang, .top, .rest, and .work where TLDs hosting domains of which around 30\% to over 50\% are bad domains. Any TLDs outside of these two lists are categorized as {\em unknown} TLDs for $F13$.}


\ignore{
{\color{orange} Here,  This `badness' index\footnote{become an expert on this, as it will be useful to your abuse paper and future studies on holistically characterizing website trustworthiness} is calculated as the ratio of the number of bad domains detected over the number of active domains observed for a particular TLD. Our list of generic TLDs contains .com, .net, .org, .xyz, .ru, .uk, .fr, .it, and .info. On the other hand, the list of abused TLDs contains .live, .buzz, .gq, .tk, .fit, .cf, .ml, .wang, .top, .rest, and .work. Any TLDs outside of these two lists are categorized as {\em unknown} TLDs. We stress that these abused TLDs are not specific to COVID-19 themed attacks. For a given TLD, we assign it a value according  to the list of generic and abused TLDs mentioned above:
0 means the given TLD belongs to the {\em generic} TLD list, 1 means the given TLD does not belong to either of the lists (indicating {\em unknown}), and 2 means the given TLD belongs to the abused TLDs list. As TLD labels produce a categorical feature, we apply one-hot encoding to create three separate binary features as F12 (TLD label 0) representing {\em generic} TLDs, F13 (TLD label 1) representing {\em unknown} TLDs, and F14 (TLD label 2) representing {\em abused} TLDs.}\footnote{rewrite this feature definition directly according to the second half of the paragraph--this seems to be the widely-used notion of binary feature; delete the first part of the paragraph. Another manifestation of "indirection/insuccinct writing"; in contrast, we need to be succinct and directly on the money, {\color{orange} Please review now and see if it is clear} {\color{red}....no, it's not, ... first, briefly review what are the three lists aim to describe, how they describe, then how we respectively leverage them to define these three features, one by one ...}} 
}
% All other TLDs, those are not in Table \ref{tab:tldList}, are labeled as `unknown'.

\item WHOIS registrar features ($F15$-$F17$):
%{\color{red}$F15$ describes ....$F16$ describes .... $F17$ describes ....}\footnote{re-organize according to this structure}

\footnote{rewrite this paragraph to directly describe what $F15$ is ...\color{orange} revised the description} {\color{orange}These feature considers the name of the website's registrar organization extracted from WHOIS. Then, we have created a list of {\em popular} and {\em bad} registrar organizations leveraging the previous study \cite{bad_registrar_list}. However, to be effective with registrar information, we need to clean up the raw data and combine similarly named registrar (e.g., Google Inc. and Google LLC.) to be identified as one registrar organization. Next, we have extracted three binary features: {\em popular}, {\em not-popular}, and {\em bad} registrars. 
%into two classes: {\em unabused} vs. {\em abused}. 
Here, feature $F15$ indicates `1' if the input website is in the {\em popular} registrars' list, and `0' if it does not appear on the {\em popular} list. Next, Feature $F16$ indicates `1' if the input website is of `not-popular' category by checking if not either in the {\em popular} registrar list or in the {\em bad} registrars list, and `0' otherwise. Lastly, Feature $F17$ indicates `1' if the input website is in the {\em bd} registrars list, and `0' if it does not appear on the {\em bad} registrar list. Our list of {\em popular} registrars contains Akamai, Alibaba, Godaddy, Google domains, Domain.com, Namecheap, name.com, CSC Corporate Domains, MarkMonitor, 1\&1, DreamHost, Hostinger,  Registrarsafe, Network Solutions, OVH, and register.com. In comparison, the list of {\em bad} registrars contains Namesilo, Dynadot, GMO, r01-ru, Nawang, Eranet, Net-Chinese, Zhengzhou, and Shinjiru \cite{bad_registrar_list}.
}
%Then, we assign it a value according to the list of popular and bad registrar organizations mentioned above: 0 means the registrar belongs to the popular registrars in the list, 1 means the registrar does not belong to the list, and 2 means it belongs to the bad bad registrars in the list. We have compiled the list of bad registrars from a previous study \cite{bad_registrar_list}. In contrast, the popular registrars' list is created by observing multiple sources of registrar reviews and registrars used by the reputed benign websites. This feature is also categorical, so one-hot encoding is applied to create binary features such as registrar\_0 (F15), registrar\_1 (F16), and registrar\_2 (F17). Our list of popular registrars contains Akamai, Alibaba, Godaddy, Google domains, Domain.com, Namecheap, name.com, CSC Corporate Domains, MarkMonitor, 1\&1, DreamHost, Hostinger,  Registrarsafe, Network Solutions, OVH, and register.com. In comparison, the list of bad registrars contains Namesilo, Dynadot, GMO, r01-ru, Nawang, Eranet, Net-Chinese, Zhengzhou, and Shinjiru \cite{bad_registrar_list}. }

\ignore{
\item Theme-based keywords ($F18$): {\color{red}This describes ....}\footnote{rewrite like how the previous ones were done ...}

\footnote{{\color{orange}This feature is not used for the detection framework, {\color{red}if so, do not call it feature and do not mention it here} but used to draw in insights hence presented it as a feature as for more data collection from generic sources keywords can be used as filters; moreover, keywords can provide us insights on the trends of attack target themes for the campaigns as a whole}} This themed Keywords are chosen keywords used for creating COVID-19 themed website names to lure in targets. This is useful as often times scammers try to bring a false sense of trust by using `test', `vaccine', `masks' keywords for similar themed scams. Hence, listing themed-keywords from the given website name is valuable. However, in this case study we are not using `keyword' as a detection feature since the dataset is already filtered with COVID-19 related keywords. Thus, using such a feature can bring overfitting problem for classifiers while using this dataset. Moreover, we aim to understand more generalized underlying structural features for malicious COVID-19 themed websites so we have not used keywords as a feature in this case study.
}
%More, obstacle with keyword feature is discussed in section \ref{sec:insights}. 
\end{itemize}

\subsubsection{Further Data Processing}

In order to collect the WHOIS information of a website (i.e., features $F1, F2, F3, F15, F16, F17$), we used the python-whois-0.7.2 library \cite{pythonWHOIS} to query the WHOIS database \cite{WHOIS_wikipedia} on 16 May, 2020.
%As part of the data processing step, we have removed all websites from our labeled dataset those do not have a \textit{WHOIS registration date} as this is one of the feature for training and 
We observe that out of the 226,000 COVID-19 themed malicious websites, {\color{orange}73,000 (or 32\%)} do not have a valid WHOIS registration lifetime information according to the query result. Moreover, out of the {\color{red}100,000}\footnote{use color to highlight these numbers that will be revised after revising the experiments} benign websites, {\color{orange}52,001 (or 52\%)} do not have the WHOIS registration lifetime information according to the query result. This prompts us to split the dataset into two with respect to the following two cases:
\begin{itemize}
\item {\color{blue}Dataset $D_1$ with WHOIS registration lifetime information (Feature $F1$)}: This dataset contains {\color{red}154,674} COVID-19 themed malicious websites and {\color{red}47,992}\footnote{this needs to be revised based on revised experiments} benign websites. {\color{red}For each website belonging to $D_1$, values of features $F1$-$F17?$ are available.}

\ignore{
{\color{red}we are talking about dataset, why jump to talk about detection framework, for which we have a subsection later? we need to modularity in writing and thinking ..} We build a unified detection framework to detect COVID-19 malicious websites with a dataset (dataset 1) of {\color{red}154,674} COVID-19 themed malicious websites and {\color{red}47,992} reputed benign websites.\footnote{delete this paragraph: it is left here for you to compare the difference between what you wrote and what i wrote ... to learn}
}


\item {\color{blue}Dataset $D_2$ without WHOIS registration lifetime information (feature $F1$)}: This dataset contains {\color{red}73,000}%\footnote{given specific number even if it's 73,000 rather than using 73K} 
COVID-19 themed malicious websites and {\color{red}52,001} benign websites. {\color{red}For each website belonging to $D_2$, values of features $F2$-$F17?$ are available (i.e., features ???? are missing).} \footnote{{\color{orange}need to check the features during re-experiments}}
\end{itemize}
By studying datasets $D_1$ and $D_2$ would allow us to draw insights into the missing of 
%This contrast study will allow us to characterize not only the effectiveness of feature $F1$ but also to what extent the missing of 
WHOIS information (i.e., {\color{red}feature $F1$}\footnote{only $F1$? should be several features, list them explicitly}) is indicative of a website being malicious.
%\footnote{think about how the latter can be done}

%A snapshot of the labeled dataset is presented in table \ref{tab:datasetDescription}. 
%Since there is more `malicious' labeled websites than `benign' labeled websites,\footnote{this is suspicious: why not simply consider top 200K, 300K, ... to add more benign website? {\color{orange}Yes, with the updated experiments we can add more from Cisco; at that time the problem was whois query takes time and querying abother 100K would take another day or two so we cut the malicious data as we still have around 100K sample which was good enough for the ML models}} for balancing the dataset we consider all `benign' labeled data and equal number of randomly selected `malicious' labeled data for feature extraction, feature selection, training, and testing of the proposed ML-based detection framework.
\footnote{delete this paragraph; it's our problem for using collecting/using enough benign websites; so we will fix the problem by collecting/using more, and enough, benign websites. this is why we need to revise the numbers related to benign websites after collecting more data and re-do the experiments ...} 

\subsubsection{Feature Selection}
\label{sec:feature_select}
{\color{orange}We propose doing feature selection before training any classifiers because that improves the classification accuracy and reducing unnecessary features actually reduces the complexity of the classifiers. we have used Pearson correlation matrix \cite{benesty2009pearson} for doing feature selection, which helps us to find more statistically independent features, and remove features which are strongly correlated (e.g., correlation coefficient > $0.60$).The feature selection is conducted with respect to datasets $D_1$ and $D_2$, respectively. First, for $D_1$, we have selected features $F1$, $F2$, $F3$, $F5$, $F8$, $F10$, $F11$, $F12$, $F14$, $F15$, and $F17$. Second, for $D_2$, we have selected features $F2$, $F3$, $F5$, $F8$, $F10$, $F11$, $F12$, $F14$, $F15$, and $F17$ \footnote{need to review this feature for this experiment when re-run experiment}

}
%\footnote{re-structure according to the above}

\ignore{
After extracting the features for all the websites, we choose the most important features and reduce the model complexity by computing the Pearson correlation  among the features. Pearson correlation helps us to find more statistically independent features, and remove features which are strongly correlated (e.g., correlation coefficient > $0.60$).\footnote{if so, we need to compare the result of doing this way vs. not doing this step; {\color{orange} We can report the accuracy improvement, but that improvement is not reported until the experiment result phase; moreover this technique is widely used in data science to reduce features as strongly correlated features create overfitting problem!}} This removal of features leads us to more accurate classification of websites and reduce the complexity of the detection framework. After analyzing the Pearson correlation and running descriptive statistical analysis, for the first experiment (experiment 1) with available WHOIS registration lifetime feature we have selected $F1$, $F2$, $F3$, $F5$, $F8$, $F10$, $F11$, $F12$, $F14$, $F15$, and $F17$ features and for the second experiment (experiment 2) without the WHOIS registration lifetime data we have selected $F2$, $F3$, $F5$, $F8$, $F10$, $F11$, $F12$, $F14$, $F15$, and $F17$ \footnote{need to review this feature for this experiment when re-run experiment}. We use these features for training and testing the proposed COVID-19 themed malicious website detection framework. Figure \ref{fig:feature_corr} shows the Pearson correlation among the selected features where lighter shade indicating weaker correlation and stronger shade indicating stronger correlation. \footnote{If we put figure \ref{fig:feature_corr} in one column I don't know how to put it in a better way with bigger fonts, but if we choose to add this in the appendix as a two-column figure then I think it's more appropriate with bigger fonts as it has no significant difference to understand the concept of the paper without looking into this figure}
}
%we randomly picked 50K `malicious' labeled websites and 50K `benign' labeled websites to generate our final dataset for the classification problem.
%\footnote{why doing this, rather than using the entire dataset? need justification {\color{orange}yes this will not the case anymore, this is a old disucssion which is added before this new updates; in our earlier dataset we had 150K malicious and 52K benign so we picked 50K 50K for two classes.}} 


%as shown in Figure \ref{fig:feature_corr} through a heat-map. This heat-map 

%\ref{fig:feature_corr}

%\subsubsection{Keyword features}
\begin{figure}[!htbp]
\centering
\includegraphics[width=1.25\linewidth]{figures/PearsonCorrelation.pdf}
\caption{Pearson Correlation Among Selected Features for $D_1$}
\label{fig:feature_corr}
\end{figure}




%\begin{insight}

%\end{insight}


%{\color {blue}[need to add some avg stats for numeric features such as avg dot counts, digit percentage among malicious and benign domains]}







\ignore{
\begin{figure}[!htbp]
\centering
\includegraphics[width=1.03\linewidth]{figures/Training_Models.pdf}
\caption{Training Phase of the Malicious COVID-19 Themed Website Detection Framework }
\label{fig:trainingmodels}
\end{figure}
}
\footnote{revise the rest like how i re-wrote the paper}

\subsection{Classifier Training}
\label{sec:detection_framework}

%\footnote{merge figure 3 and 4 into a single picture, {\color{orange}Ok I will add them together}}


In this case study, we propose a COVID-19 themed malicious website detection framework using multiple Machine Learning classifiers, including the majority voting based ensemble learning classifier, to find the best-fitted model for the detection. We have leveraged Random Forest, Decision Tree, Logistic Regression, and K-Nearest Neighbor \footnote{we can add more when re-run experiment like gradient boosting}, as ML classifiers and include the ensemble learning for our detection framework. Figure \ref{fig:detectionFramework} presents the framework, where we split the labeled dataset by 80/20 for training and testing the classifiers, respectively. All the selected features for associated dataset in section \ref{sec:feature_select} and the labels extracted for websites of the 80\% training dataset are input to the classifiers to train themselves. Once the classifiers are well trained, we run the testing module of the framework. We evaluate the individual classifiers for predicting the website labels of the 20\% testing dataset. Notably, as there is no duplication in the dataset, hence the testing data is entirely unseen for the framework during training. Thus, training on the list of retrospect websites until $(t-1)$-th day and using the trained classifiers for detecting the COVID-19 themed malicious websites on the $t$-th day is a feasible model build for real-time detection of COVID-19 themed malicious websites going forward. 

%Figure \ref{fig:trainingmodels} depicts the architecture for the training of $C_1 \dots C_K$ ML classifiers based on the selected features for the input websites as training data. Again, Figure \ref{fig:predictionFramework} presents the majority voting-based ensemble learning prediction framework given a list of \textit{unlabeled} COVID-19 domains on the $t$-th day as input. The output of this framework is 
%the likeliness of COVID-19 domains (test data) being malicious 
%the predicted malicious COVID-19 domains (from test data) on the $t$-th day. Now, suppose the $j$-th classifier ($C_j$) predicting the $i$-th domain's ($d_i$) label is presented by $c_{i,j}$. Hence, 
%{\color{red}[need to add a updated figure for training and testing workflow and description]}

\subsubsection{Majority Voting Based Ensemble Learning}
Instead of depending on one particular ML classifier ensemble learning classifier usually aggregates and incorporates outputs from multiple ML classifiers to provide more accurate and trustworthy classification outcome. Here in this case, suppose, there are $K$ number of individual classifiers which are contributing to the ensemble learning classifier. If the prediction label of the $j$-th classifier, $C_j$, predicting the $i$-th website is presented by $x_{i,j}$. Then, the majority voting based ensemble learning classifier's prediction label, $l_i$, for the $i$-th website can be outlined as equation \ref{eq:ensembleVoting}. 
\begin{eqnarray}
\label{eq:ensembleVoting}
l_i=\left\{
\begin{array}{ll}
1     & \sum_{j=1}^{K} x_{i,j} > K/2 \\
0     & Otherwise
\end{array}
\right.
\end{eqnarray}

Here, the prediction label $l_i$ = 1 if the majority of the ML classifiers are predicting the $i$-th website as malicious, otherwise $l_i$ = 0 if majority of the ML classifiers are predicting the $i$-th website as benign or there is a tie between the classifiers. 



%\begin{eqnarray}
%l_i=\left\{
%\begin{array}{ll}
%1     & , w_i:= malicious\\
%0     & , w_i:= benign
%\end{array}
%\right.
%\end{eqnarray}


%\begin{equation}
%    l_i = \sum_{j=1}^{K} c_{i,j} \geq K/2
%\end{equation}



\ignore{
\begin{figure}[!htbp]
\centering
\includegraphics[width=1.04\linewidth]{figures/Prediction_Framework.pdf}
\caption{Testing Phase of the Malicious COVID-19 Themed Website Detection Framework}
\label{fig:detectionFramework}
\end{figure}
}

\subsection{Experiments and Results}

\subsubsection{Performance Metrics}
We propose adopting standard metrics to measure a detector's performance: accuracy (ACC), false-positive rates (FPR), false-negative rates (FNR), and AUC score \cite{???}. 
Specifically, let $TP$ be the number of true positives, $TN$ be the number of true negatives, $FP$ be the number of false positives, and $FN$ be the number of false negatives. Then, we have
$ACC = \frac{TP + TN}{TP + TN + FP + FN}$, 
$FPR = \frac{FP}{FP + TN}$,
$FNR = \frac{FN}{FN + TP}$, and
%$DR = \frac{TN}{FP + TN}$
{\color{red}$AUC=?????$}
\footnote{{\color{orange} need to provide equation for AUC score or cite source}}


\subsubsection{Experiment Design}

{\color{orange}To analyze both the context of dataset $D_1$ and $D_2$, we are proposing to conduct the following experiments.
\begin{itemize}
\item Experiment-1: This experiment considers the COVID-19 themed malicious and reputed benign websites with the available WHOIS registration life-time ($F1$) feature. With this we want to analyze what impact $F1$ feature has over the performance of the detection framework. To conduct the experiment we train the detection framework proposed in section \ref{sec:detection_framework} with randomly selected 80\% training dataset {\color{red}(?? malicious and ?? benign}\footnote{need to add these numbers after re-experiments}) from $D_1$ and use the rest 20\% of $D_1$ {\color{red}(?? malicious and ?? benign)} to test the framework.   
\item Experiment-2: This experiment considers the COVID-19 themed malicious and reputed benign websites without the available WHOIS registration life-time ($F1$) feature. This contrast experiment (Vs Experiment-1) is actually helping us analyze the impact of feature $F1$ over the performance of the detection framework and also indicating what other features can detect the malicious website if $F1$ feature is not present. In this experiment we train the detection framework proposed in section \ref{sec:detection_framework} with randomly selected 80\% training dataset {\color{red}(?? malicious and ?? benign)} from $D_2$ and use the rest 20\% of $D_2$ {\color{red}(?? malicious and ?? benign)} to test the framework.  

%\item RQ3: ...
\end{itemize}

%Each research question will be investigated using datasets $D_1$ and $D_2$.

%\subsubsection{Answering RQ1}
\subsubsection{Results for Experiment-1}
%The 20\% test data of $D_1$ consists of {\color{red}9,962 benign and 11,633 malicious websites}\footnote{numbers need to be reviewed after the re-experiment}. 
With the above mentioned experiment setup we measure the performance of independent ML classifiers and the majority voting based ensemble learning framework as shown in table \ref{tab:MLClassifierPerformance}. The results show {\color{red} that the Random Forest classifier outperforms other ML classifiers for detecting COVID-19 themed malicious websites with 97.7\% accuracy. Moreover, the Random Forest (RF) classifier has only around 4\% FPR and 0.84\% FNR with an AUC score of 0.988, which is the best compared with other classifiers. Interestingly, the performance of the ensemble learning classifier is not outperforming the RF classifier as we hypothesized while designing the framework architecture and it is at best showing similar performance as the RF model. Moreover, in figure \ref{fig:ROCCurve} we also plot the ROC curve for individual classifiers to show the robustness of those classifiers in effectively detecting COVID-19 themed malicious websites.}\footnote{This result section will be updated with ew-experiment results}    

\subsubsection{Results for Experiment-2}
%In this experiment the 20\% test data of $D_2$ consists of {\color{red}?? benign and ?? malicious websites}\footnote{numbers need to be reviewed after the re-experiment}. 
With the above mentioned experiment setup for experiment-2, we measure the performance of independent ML classifiers and the majority voting based ensemble learning framework as shown in table \ref{tab:MLClassifierPerformance_ex2}. The results show {\color{red} that ....}\footnote{This result section will be updated with ew-experiment results}  

}
%For answering RQ1 with respect to dataset $D_1$, we conduct the following experiment ... The experiment result is summarized as follows ...
\ignore{
{\color{red}
For answering RQ1 with respect to dataset $D_2$, we conduct the following experiment ... The experiment result is summarized as follows ...

\subsubsection{Answering RQ2}

%For answering RQ2 with respect to dataset $D_1$, we conduct the following experiment ... The experiment result is summarized as follows ...

For answering RQ2 with respect to dataset $D_2$, we conduct the following experiment ... The experiment result is summarized as follows ...

\subsubsection{Answering RQ3}

For answering RQ3 with respect to dataset $D_1$, we conduct the following experiment ... The experiment result is summarized as follows ...

For answering RQ3 with respect to dataset $D_2$, we conduct the following experiment ... The experiment result is summarized as follows ...
}
}
\footnote{re-structure the rest of the section according to the preceding ... we need to have a logically meaningful way of thinking:  problem $\to$ experimental design $\to$ experimental result ...}


%\subsubsection{Experiment-1}
%In this experiment we consider the malicious and benign websites with the available WHOIS registration life-time feature. We use the detection framework proposed in section \ref{sec:detection_framework} to test with the 20\% testing data from dataset 1, which consists of {\color{red}9,962 benign and 11,633 malicious websites}\footnote{numbers need to be reviewed after the re-experiment}. We measure the performance of independent individual ML classifiers and the majority voting based ensemble learning framework as shown in table \ref{tab:MLClassifierPerformance}. The results show that the Random Forest classifier outperforms other ML classifiers for detecting COVID-19 themed malicious websites with 97.7\% accuracy. Moreover, the Random Forest (RF) classifier has only around 4\% FPR and 0.84\% FNR with an AUC score of 0.988, which is the best compared with other classifiers. Interestingly, the performance of the ensemble learning classifier is not outperforming the RF classifier as we hypothesized while designing the framework architecture and it is at best showing similar performance as the RF model. Moreover, in figure \ref{fig:ROCCurve} we also plot the ROC curve for individual classifiers to show the robustness of those classifiers in effectively detecting COVID-19 themed malicious websites.    
%\subsubsection{Experiment-2} 
%In this experiment we consider the malicious and benign websites without the available WHOIS registration life-time feature. We use the same detection framework proposed in section \ref{sec:detection_framework} to test with the 20\% testing data from dataset 2, which consists of {\color{red} ?? benign and ?? malicious websites}\footnote{numbers need to be added after the re-experiment}. The performance of the detection framework for this experiment is shown in table \ref{tab:MLClassifierPerformance_ex2} \footnote{{\color{orange}need to generate another table for performance of experiment 2}}.
%{\color{orange}(we can discuss the performance after the experiment here)}
%along with majority voting based ensemble learning model. ....

\begin{table} [!htbp]
  \caption{Performance of the Detection Framework for Experiment-1}
  \label{tab:MLClassifierPerformance}
  \begin{tabular}{|c|c|c|c|c|}
    \toprule
    ML Classifiers & ACC & FPR & FNR & AUC Score\\
    \midrule
    RF & 97.70\% & 4.01\% & 0.84\% & 0.988 \\
    DT & 96.82\% & 3.80\% & 2.65\%& 0.976 \\
    KNN  & 97.24\% & 5.31\% & 0.58\% & 0.983 \\
    LR & 97.51\% & 5.4\% & 0\% & 0.981 \\
    Ensemble Learning & 97.69\% & 4.03\% & 0.84\% & 0.976\\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table} [!htbp]
  \caption{Performance of the Detection Framework for Experiment-2}
  \label{tab:MLClassifierPerformance_ex2}
  \begin{tabular}{|c|c|c|c|c|}
    \toprule
    ML Classifiers & ACC & FPR & FNR & AUC Score\\
    \midrule
    RF & ??\% & ??\% & ??\% & ?? \\
    DT & ??\% & ??\% & ??\%& ?? \\
    KNN  & ??\% & ??\% & ??\% & ?? \\
    LR & ??\% & ??\% & ??\% & ?? \\
    Ensemble Learning & ??\% & ??\% & ??\% & ??\\
    \bottomrule
  \end{tabular}
\end{table}


\ignore{
\begin{figure}[!htbp]
\centering
\includegraphics[width=1.24\linewidth]{figures/PR_AUC_curve.pdf}
\caption{PR-AUC Curve for Different Classifiers {\color{red}legend fonts too small; curves should have the same thickness}}
\label{fig:pr_AUC_curve}
\end{figure}
}

\begin{figure}[!htbp]
\centering
\includegraphics[width=1.04\linewidth]{figures/ROC_curve.pdf}
\caption{ROC Curve for Different Classifiers {\color{red}Will update this figure with bigger fonts for x-label and y-label}}
\label{fig:ROCCurve}
\end{figure}

\subsection{Interesting Insights and Research Questions from COVID-19 Themed Malicious Website Datasets}
\label{sec:insights}
After extracting the features for websites in our final preprocessed dataset, we try to look deep and find insights by investigating from COVID-19 themed Vs. non-COVID-19 themed website perspectives. We analyze the data through statistical analysis and visualizing the trends for the data.

At first, we check the number of websites each day since February 1, 2020, reported by the {\color{red}two} three datasets, as shown in figure \ref{fig:website_trend}. %Here, Malware Patrol COVID-19 dataset \cite{COVID19_data_malPatrol} has no data point reported before March 1, 2020. 
If we look closer into the trend of the graphs, we observe that COVID-19 related new domain registration has been decreasing from late March 2020, giving us the following insight. 

\begin{insight}
Most of the COVID-19 themed websites were created during the early stage of a pandemic (within the first three weeks from March 11, 2020) when people had little knowledge and preparation on the volume of the coming cyber attacks. As days passed, more defense and detection mechanisms were applied, resulting in a downward graph of newly registering COVID-19 themed websites. 
\end{insight}

However, it will be interesting to see if this trend goes up on the later stages of the pandemic when vaccines and therapeutic researchers would get results at their hands. As we are going through an unprecedented time, we may still uncover new insights going forward. It will be interesting to answer research questions like \textbf{\textit{RQ1:} Given relevant data, can we correlate the downward trends of COVID-19 themed domain registration with upward trends of any other themed malicious domains during this pandemic}? Answering \textit{RQ1} may give us insight that attackers are using constant efforts. However, they change the target theme of their efforts based on success probability. 

\begin{figure}[!htbp]
\centering
\includegraphics[width=1.04\linewidth]{figures/trend_analysis_chart.pdf}
\caption{COVID-19 themed website trends {\color{red}(need to remove malware patrol data)}}
\label{fig:website_trend}
\end{figure}

Next, we try to understand the quality of our COVID-19 themed website dataset. We see that Malware Patrol and Domain Tools COVID-19 dataset show more consistency in the daily number of newly registered COVID-19 themed websites than the CheckPhish COVID-19 dataset \ref{fig:website_trend}. One of the reasons might be the collection mechanism, as CheckPhish mentions the inclusion of users' reported scam websites (or URLs) on their COVID-19 feeds, which may vary on different days. These datasets also bring the valid research question, \textbf{\textit{RQ2:} How good is the ground-truth data, can we evaluate the quality of these feeds (or other COVID-19 feeds) and identify the actual false positives and false negatives?} Answering \textit{RQ2} may help us build better detection and prediction models in the future as ground-truth data scarcity, for labeling `benign' COVID-19 themed websites, which is a real pain point. Moreover, we have also observed in our COVID-19 themed combined (both `malicious' and `benign') dataset reported until May 15, 2020, around 7\% of websites had WHOIS registration date before December 1, 2019, which was before the official date of the first COVID-19 case. We are assuming that they are in the dataset because of using specific keywords such as `vaccine', `test', and`mask' keywords; otherwise, they are government hosted websites with country-level TLDs (e.g., .ar for Argentina) hosting legit COVID-19 contents. Nevertheless, these assumptions are non-conclusive with further extensive experiments.  

Next, we observe the registrar distribution to discover the top 10 registrars for COVID-19 themed websites and their corresponding percentage with the Cisco top websites, as depicted in figure \ref{fig:registrarDistribution}. It shows that most bad guys are leveraging cheap domain registration and `shared hosting' \cite{zero_day_mal_ip} options. For example, a percentage of 1\&1 and Google domains as registrar for the COVID-19 themed website vs. the top Cisco website are alarming. This analysis has further lead us to the following insight.   


\begin{figure}[!htbp]
\centering
\includegraphics[width=1.10\linewidth]{figures/chart_registrar.pdf}
\caption{Distribution of registrars for COVID-19 related websites}
\label{fig:registrarDistribution}
\end{figure}


\begin{insight}
Registrar information could be vital in detecting and predicting COVID-19 themed websites. An enterprise may think about being skeptical and suspicious about certain registrars during this pandemic. 
\end{insight}

%\begin{insight}
%Attackers are leveraging cheap `shared hosting' options for registering attack domains. A previous study found that shared hosting is a soft target for malicious content (e.g., IP address, domains) hosting \cite{zero_day_mal_ip}.    
%\end{insight}


Next, we observe the distribution of TLDs to find the top 10 TLDs among COVID-19 websites Vs. their corresponding percentage in Cisco top websites, as shown in figure \ref{fig:tldDistribution}. Though `.com' is the topping the list with a far higher number of TLDs if we look closely at the percentage we may see `.org', `.info', and `.uk', these TLD have more abused percentage when compared with Cisco's top websites. We also observe 8 out of the top 10 TLDs of Cisco top websites are also presented in COVID-19 themed top 10 TLDs except the `.io' and `.cn', which gives us the following insight.

\begin{insight}
Attackers are using popular TLDs to evade traditional historically abused TLD-based security detection during this COVID-19 pandemic. However, knowledge of percentage of abuse by a generic TLD provides as an effective detector for COVID-19 themed malicious websites.   
\end{insight}

\begin{figure}[!htbp]
\centering
\includegraphics[width=1.02\linewidth]{figures/chart_tld.pdf}
\caption{Distribution of top-level-domains (TLDs) for COVID-19 themed Vs. overall dataset}
\label{fig:tldDistribution}
\end{figure}

Next, we extract the keywords from the website domain names in our dataset by splitting connected words using python Word Ninja library \cite{python_wordninja} along with an updated language model. In this new language model, we heuristically accommodate COVID-19 related words (e.g., quarantine, testing) in earlier ranks than the original 125k Wikipedia English language model. Extracting keywords gives us the following insight on keyword trends.  

\begin{insight}
The top 15 popular and meaningful keywords for COVID-19 related domain names are `covid', `corona', `covid19', `coronavirus', `mask', '19', 'masks', `quarantine', `virus', `test', `facemask', 'pandemic', 'face', and `vaccine' as per our COVID-19 themed website dataset. 
\end{insight}

However, Word Ninja is not 100\% perfect as the accuracy of splitting depends on the input language model which brings future research opportunity such as, \textbf{\textit{RQ3:} How can we develop more accurate language model for detecting COVID-19 themed keywords?} This keyword extraction process has led us to another exciting insight.

\begin{insight}
While most of the websites are named in the English language, there are COVID-19 themed websites in our dataset that use English characters but represent Spanish, Russian, or Indian language meanings. Thus using the keyword as features may not be a good fit before finding language-specific keywords and meaning to reduce model errors or biases.  
\end{insight}

Next, we also investigate a list of COVID-19 themed websites targeting to lure users from a particular geographical region (e.g., Texas state). We have found that  `coronaviruspreventionsanantonio.com', `coronavirusprecentionhouston.com', and `coronaviruspreventiondallas.com', %`covid-19preventionsanantonio.com', `covid-19prevention-houston.com', and `covid-19preventiondallas.com' 
are using the same information and contents with different look and feel (e.g., changing the CSS template). All these domain names are using city names and COVID-19 keywords as lures. We could not verify the maliciousness of those domains as they represent a Texas-owned local business `rpmtexas.com'. However, this finding gives us the following insights.  

\begin{insight}
The same HTML content might be reused among different domains to reduce costs and reach more victims.  
\end{insight}


\begin{insight}
Attackers may use city name and combine with COVID-19 keywords to register new websites and lure victims in a targeted geographical region. 
\end{insight}



%Precision recall Curve is shown as alternative to ROC curve as we are working with an imbalanced dataset \cite{Precision_Recall_curve_VS_ROC_curve, Saito2015ThePP}. 

%Next, we measure the same performance metrics for a new unseen set of domains that are registered (and published) after May 15, 2020 through Malware Patrol repository. We observe that our model is performing quite well to predict zero-day (previously `unseen') malicious COVID-19 domains. Table \ref{tab:MLClassifierPerformance_zeroDay} highlights the perform ace of our prediction framework over a set of previously unseen domains.   


==> methodology.tex <==
Figure \ref{fig:researchSteps} highlights our methodology, which has three steps. The firs step is to characterize the COVID-19 themed cyber attacks from various perspectives, such as: what the attackers do, what the attackers exploit, how the attackers exploit, and what the attackers attempt to accomplish, what sectors are targeted by the attackers. These understandings allow us to map the attacks into a cyber threat framework, such as the Cyber Kill Chain \cite{lockheedMartin_killchain}. This allows us to get an even more systematic understanding of the attackers' techniques, evading strategies, attack patterns, and attack goals. 

\ignore{
%, and transmission medium of attacks.
%{\color{red} Min's comment : If we are going to remove the recommendation section, we need remove step 4:} \textbf{Resolved} 
\begin{figure}[!htbp]
\centering
\includegraphics[width=1.02\linewidth]{figures/research_steps.pdf}
\caption{The research methodology {\color{red}merge the mapping into cyber kill chain into step 1, as it belongs to section 3}}
\label{fig:researchSteps}
\end{figure}
}

The second step is to design defences strategies against COVID-19 themed attacks. {\color{blue}... add something  here to summarize what section 4 does ...}

%Next, in the fourth step we provide general guidelines and recommendations for similar future attacks and/or attacks during similar future events of crisis. In this step, we summarize the experts recommendations from both academia and industry to fight against unprecedented volume of cyber attacks during this pandemic given scenarios like `stay-at-home' order in place or not. 

Finally, in the fifth step, we show a case study on the effectiveness of our defense mechanism while fighting against the unseen COVID-19 themed malicious websites. We show how effectively we can classify those new malicious websites from benign ones, before they are dispatched to the users for attach such as phishing, malware propagation, social engineering, selling fraud products or services, and scamming. 
%This case study is performed to evaluate the effectiveness of our defences and shows the fact that a change in feature parameters of day-to-day detection frameworks need to be adjusted to catch COVID-19 themed attacks (or any future global event-themed attacks). 

%In this paper we are highlighting five high level problems which is indicated as individual research steps as shown in Figure \ref{fig:researchSteps}. In the very firs step, we study already reported COVID-19 cyber attacks and social engineering attacks to characterize these attacks according to their attack types,  target industries, and transmission medium of attacks. Here, attack types include what attackers do, what they exploit, how they exploit, and what they are achieving (or trying to achieve), In the next step, we try to map these attacks into the Cyber Kill Chain threat framework for following reasons- i) Get a bird's eye view of the situation on attacker's techniques and evading strategies, ii) Get an overall idea of attack patterns or campaigns and their level of advancement, iii) Understand high level attack goals of the attackers to penetrate a humanitarian crisis situation (such as, COVID-19 pandemic). In step 3, we design and discuss both state-of-the-art and new defences based on our findings in step 2 that we believe are effective against the various attacks we identified in step 1. The following step (step 4) provides general guidelines and recommendations for similar future attacks and/or attacks during similar future events of crisis. In step 4, we summarize the experts recommendations from both academia and industry to fight against unprecedented volume of cyber attacks during this pandemic. Finally, in step 5 we show a case study on predicting malicious domain names before they are dispatched to the users for phishing, malware propagation, social engineering, selling fraud products or services, and scamming attacks. This case study is performed to evaluate the effectiveness of our defences and shows the fact that a change in feature parameters of day-to-day detection frameworks need to be adjusted to catch COVID-19 themed attacks (or any future global event-themed attacks). 



==> recommendation-outdated.tex <==

In this section, we summarize the experts' recommendations provided by industry leaders and our independent tips on maintaining cyber hygiene and continuing business securely during this pandemic and similar future crisis. We provide a separate set of recommendations for enterprise-level security with and without active `shelter-in-place' (or `stay-home') orders. 

%{\color{blue} We also discuss the feasibility and importance of executing recommended actions in organizations based on their sizes?}

\subsection{Recommendations from industry experts}
Experts from VMware Carbon Black, a top giant in the cybersecurity industry, have published a webinar discussion where they metaphorically presented ``digital distancing" as equivalent to ``social distancing" while fighting against the unprecedented cyberattacks during this pandemic \cite{CBDigitalDistancing}. They bring the fact that many of our smart IoT devices at home are unpatched and more than 70\% percent of employees are working remotely as per WFH policy, they are making the enterprise network vulnerable by increasing the attack surface that is not in sight of any security teams. Given these facts, to practice ``digital distancing", Carbon Black suggested to setup routers with two separate networks. This approach can isolate our enterprise networks from the unchecked home devices with enforced limited privileges and thus significantly reduce the attack surface. This webinar session also highlighted how to practice organizational security hygiene by 1) using passwords for changing application settings, 2) passwords for remote meetings, 3) whitelisting applications, 4) deliver security updates outside of corporate networks, 5) communicate new risk factors to employees and customers 6) provide timely tips to secure home networks during remote work \cite{CBDigitalDistancing}. They even suggested using threat hunting strategies in-home network environments if remote working becomes the ``new-normal".
Moreover, another cybersecurity expert, Rick McElroy, from VMware Carbon Black, recommended three necessary steps as equivalent to ``washing your hands for the 20 seconds." to protect enterprise security. He suggested patching and regular updating software, using multi-factor authentication (MFA), and leveraging virtual private network (VPN) as the three primary steps for all organizations that have shifted to the remote work model. Other organizations are also suggesting tightening security with the use of MFA and VPNs \cite{CBWashingHand20s}. However, experts also discussed that VPN alone would not be enough, and large scale use of VPNs may provide enough incentives to attackers for targeting VPN's vulnerabilities \cite{CyberHyigene_during_COVID19}. Experts suggest that train employees are still one of the most effective ways to fight against these large number of attacks. Thus, early warnings and communications about similar attack scenarios and implementing policies on what to do with such COVID-19 related emails should be in place \cite{CyberHyigene_during_COVID19}. Experts suggests that this pandemic might be a perfect scenario for enabling zero trust model for sensitive data access. To sump up, experts suggested to have a solid and immediate incident response plan if a COVID-19 related security breach happens during this pandemic.


%avoid online viruses by virtual social distancing: (don't right away believe what you see or read, it may be a misinformation, check source, check publish date, search other media that publishes similar story...) report in https://siliconangle.com/2020/04/03/cyber-hygiene-in-the-time-of-covid-19-avoid-catching-an-online-virus-by-virtual-social-distancing-cubeconversations/


\subsection{Recommendations while `stay-at-home' orders in place}
Since COVID-19 disease has no vaccination yet, to slow down the infection rate, `stay-at-home' order has been the most effective way to allow health systems to treat COVID-19 patients without overwhelming their resources. Thus, while assessing the security plans for business continuity, we need to keep in mind that work from home (WFH) is not going away soon. Hence, policies and clear guidelines should be established to set up for a secure remote work environment. Here we recommend some of the technical safeguards and policy design while `stay-home' orders are active during a crisis. 
%\subsubsection{Technical safeguards}
While experts are suggesting VPN as a safeguard, but organizations should create a list of approved and reputed VPN software so that users do not fall victim to attractive VPN lures. Similarly, they should provide clear direction on which remote tools and remote meeting software to use while accessing enterprise networks from home. These whitelisting of applications would provide more visibility from the defenders' perspective. All remote meetings should be password protected to avoid any eavesdropping and should have an admin who allows other valid participants to join meetings when requested. Next, an enterprise should provide employees with work laptops at home to have all the essential standard tools in that machine readily available. This policy reduces the attack surface significantly, which is created while using their home laptops and installing unchecked vulnerable third-party software.   
An organization should provide specific guidelines for employees and consumers to securely access data and networks remotely. Another essential advice is to strengthen the remote access policies of the enterprise as remote working might be a ``new normal" for the rest of this year 2020. We suggest using a coordinated hybrid approach for security and logs monitoring with automation, machine learning, and human analysts to fight against the large number of attacks.

\subsection{Recommendations independent of the `stay-at-home' orders}
Though `stay-at-home' is the reality in the current situation for many tech companies, COVID-19 attacks may stay even when the stay-at-home orders are lifted. Mass campaigns with email lures, building \& registering malicious domains, creating malicious mobile applications can still impact the businesses which are already hardly impacted economically. Hence to be resilient during this crisis (or similar future events) we recommend practicing standard cyber hygiene and proactive defense strategies for a much more extended period even when `stay-at-home' order is not in effect. 

%\subsubsection{Technical safeguards}
This pandemic should give the enterprise leaders a strong message to strengthen security monitoring, proactive defense, and test security software effectiveness regularly. The proactive defense should include defending against new website abuses, new malicious domains, and IP addresses, predicting known attack groups from real-time incident reports and security logs, scanning of emails with newly registered COVID-19 related links, and attachments related to COVID0-19 lures. Enterprises should be proactive and ready to change their existing models and frameworks to detect these attacks effectively. Furthermore, security teams should work with fraud management and risk management teams to facilitate better detection, monitoring, and response and coordinate with decision-makers to facilitate compact incident response plans. 

%\subsubsection{Awareness safeguards} 
Moreover, enterprises should actively communicate these risk factors and attack scenarios to train their employees and users. Primarily, organizations should warn their employees to be skeptical about COVID-19 related emails with links and attachments from the company’s CEO or their doctors with COVID-19 advice and guidelines. All enterprises should communicate their employees on how often and who are going to send emails regarding COVID-19. Employees should be trained not to open suspicious emails, not to click on attachments or links, and know the steps on what to do or whom to notify when they encounter such an email. Suspicious emails may use COVID-19 lures (mentioned in section 3) to emotionally distressed employees with compassionate sentences to become successful. The first wall of defense is the human shield, as most of the attacks need human interaction and error to be victorious. Everyone should always double-check the sender's address for COVID-19 emails. To avoid fraud donations, instead of making payments from email links, we should go to the website where we want to donate. Enterprises should teach their employees on hidden email links and how hovering over a link can discover the real website (or domain address). We should no download untrusted third-party VPN, remote access, and virtual meeting software. One way to maintain cyber hygiene is to check reviews of software and discuss new tools among peers, which may save individuals and enterprises from potential risks. Always check for the reliable and original source for news and COVID-19 updates. Double-checking website addresses may protect individuals from visiting a phishing website or downloading a malicious piece of software. We should not share sensitive news or videos on social media before confirmation from reliable sources, as this might ponder violence. We should not buy or trust testing kit, vaccines, therapies, cures from unreliable sources that are not approved by national or international level health agencies.



==> recommendations.tex <==

This section summarizes the experts' recommendations provided by industry leaders and our independent tips on maintaining enterprise security, privacy regulation compliance and business continuity during this pandemic and similar future extended period of business disruption. We compile a separate list of recommendations based on `stay-at-home' (or WFH policy) orders in effect or not.
%{\color{blue} We also discuss the feasibility and importance of executing recommended actions in organizations based on their sizes?}

%\subsection{Recommendations from Experts Regarding Remote Work}

\subsection{Recommendations Regarding Remote Work}
Since COVID-19 disease has no vaccination yet, to slow down the infection rate, stay-at-home orders along with social distancing have been the most effective ways to allow health systems to treat COVID-19 patients without overwhelming their resources \cite{Stay_home_covid19}. Thus, while assessing the cybersecurity plans for business continuity, enterprises need to keep WFH policy in mind. During active WFH policy enterprises should publish clear guidelines for their remote employees. The following recommendations can guide the community to chose from according to their budgets and valuation of assets. 
%\subsubsection{Secure home networks}
\subsubsection{Secure home-work environments}
\begin{recommendation}
Practice ``digital distancing" by setting up routers with two separate networks, isolate enterprise networks from unpatched home devices  \cite{CBDigitalDistancing}.
\end{recommendation}

\begin{recommendation}
Enterprises should provide tips to secure home networks and deliver security updates outside of corporate networks \cite{CBDigitalDistancing}.
\end{recommendation}

\begin{recommendation}
Provide employees with work laptops at home to have all the essential standard tools in that machine readily available, it can protect enterprises from reducing attack surfaces created by unverified and unchecked third-party software installations at employee's end. 
\end{recommendation}

\begin{recommendation}
\label{rec:dnsSettingsPass}
Provide guidelines for employees and customers to use stronger passwords for PCs and routers, regularly monitor DNS settings. 
\end{recommendation}

\begin{recommendation}
Build capabilities of enterprise threat hunting within employee's home network environments \cite{CBDigitalDistancing}.
\end{recommendation}
\subsubsection{Do not neglect employee information and privacy}
\begin{recommendation}
Record only factual information and  minimum amount of information necessary. 
\cite{Addiscott2020}.
\end{recommendation}
%disucssion points
%Experts from VMware Carbon Black, a top giant in the cybersecurity industry, have published an on-demand webinar discussion where they metaphorically presented ``digital distancing" as equivalent to ``social distancing" while fighting against the unprecedented cyberattacks during this pandemic in the digital world . 
%They bring the fact that many of our smart devices at home are unpatched. While 80-90\% percent of employees are working from home, they are making the enterprise network vulnerable by increasing the attack surface that is not in sight of any security teams. Given these facts they recommends the following to reduce the attack surface.

\subsubsection{Secure remote communication}
\begin{recommendation}
Always use passwords and restrict user joining meetings by admin verification for remote meetings to avoid any eavesdropping \cite{CBDigitalDistancing}. 
\end{recommendation}

\begin{recommendation}
Do not use keywords such as `sensitive', `secret', `highly-classified' as meeting titles \cite{CBDigitalDistancing}.
\end{recommendation}

\begin{recommendation}
Leveraging virtual private networks (VPN) for remote access to enterprise network while working from home \cite{CBWashingHand20s}.
\end{recommendation}

\begin{recommendation}
\label{rec:mfa}
Using multi-factor authentication (MFA) for all critical communications and transactions \cite{CBWashingHand20s}. (more citations) 
\end{recommendation}

%The session also recommended to practice organizational security hygiene as listed below -
\subsubsection{Build more informed users}
\begin{recommendation}
Enterprise should specify a (or make a white-list) VPN software and remote access tools for their employees which may prevent them falling into VPN lure traps.
\end{recommendation}

\begin{recommendation}
Provide clear direction for remote meeting software and meetings norms while working from home.
\end{recommendation}

\begin{recommendation}
Enterprise should provide specific guidelines for employees and consumers to securely access data and networks remotely.
\end{recommendation}


%Next, another cybersecurity expert from VMware Carbon Black, recommended three necessary steps as equivalent to ``washing your hands for the 20 seconds" to protect enterprise security \cite{CBWashingHand20s}. These steps are listed as the next three subsequent recommendations below. 
%These same set of recommendations are also coming from other security experts and farms \cite{}. The steps are listed below as individual recommendations. 







%Experts suggest that train employees are still one of the most effective ways to fight against these large number of attacks. Thus, early warnings and communications about similar attack scenarios and implementing policies on what to do with such COVID-19 related emails should be in place \cite{CyberHyigene_during_COVID19}.


%Finally, experts suggests enterprises to have a compact and immediate incident response plan if COVID-19 related security breach happens during this pandemic.



%avoid online viruses by virtual social distancing: (don't right away believe what you see or read, it may be a misinformation, check source, check publish date, search other media that publishes similar story...) report in https://siliconangle.com/2020/04/03/cyber-hygiene-in-the-time-of-covid-19-avoid-catching-an-online-virus-by-virtual-social-distancing-cubeconversations/


%\subsection{Recommendations on enterprise security while `stay-at-home' orders in place}
%\subsubsection{Technical safeguards}


%These whitelisting of applications would provide more visibility from the defenders' perspective. 






%Another essential advice is to strengthen the remote access policies of the enterprise as remote working might be a ``new normal" for the rest of this year 2020. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Recommendations from Experts Independent of Remote Work}
\subsection{Recommendations Independent of Remote Work}
Though WFH policy is the actual reality in many industries at current situation, COVID-19 themed attacks may stay even longer after the stay-at-home orders are lifted. 
%Mass campaigns with email lures, building \& registering malicious domains, creating malicious mobile applications can still impact the businesses which are already hardly impacted economically. 
Hence to be resilient during this crisis and future similar themed cyberattacks there is no other alternative than practicing standard cyber hygiene, be vigilant, and establish more proactive defense strategies. The list of recommendations are as follows.

\subsubsection{Secure end-points}
%Thus enterprises need guidelines for secure business continuity to fight this pandemic from both health and economic perspectives.  
\begin{recommendation}
Timely patching and updating of all software and operating systems \cite{CBWashingHand20s}.
\end{recommendation}


\subsubsection{Secure networks \& systems}
\begin{recommendation}
Using mandatory passwords for changing any application settings, if working with sensitive infrastructures, system level whitelisting of applications can be practiced \cite{CBDigitalDistancing}. 
\end{recommendation}

%\subsubsection{Improve security practices}


%\subsubsection{Secure }
\begin{recommendation}
Establish proactive defense against COVID-19 related malicious and abused websites, domains, URLs, and IP addresses.
\end{recommendation}

\begin{recommendation}
Establish proactive defense against COVID-19 themed malicious emails through scanning and reviewing emails with COVID-19 related subject, body, links, and attachments before sending it to employee's inbox.  
\end{recommendation}

\subsubsection{Build more informed users}
\begin{recommendation}
Enterprise should establish a secure communication channel either through email or web portal for reliable COVID-19 related information and updates, try to boost employee morale by showing more connection and compassion.  
\end{recommendation}

\begin{recommendation}
\label{rec:awareOnlure}
Establish an effective way to regularly communicate about new COVID-19 related lures, misinformation, myths, and risk factors to employees and customers to educate them beforehand \cite{CBDigitalDistancing}.
\end{recommendation}

\begin{recommendation}
Train employees to be skeptical and vigilant about emails with COVID-19 related updates, information, guidelines, or about ongoing sales or deals.
\end{recommendation}

\begin{recommendation}
Encourage and provide guidelines for employees and customers to report about any suspicion, scams, or abuses to IT (or security) teams.   
\end{recommendation}

%\begin{recommendation}
%Organizations should warn their employees to be skeptical about COVID-19 related emails with links and attachments from the company’s CEO, personal doctors with COVID-19 advice and guidelines, or emails pretending to be deals/offers from legit retailers. \cite{}
%\end{recommendation}


%\begin{recommendation}
%Employees should be trained not to open suspicious emails, not to click on attachments or links, and know the steps on what to do or whom to notify when they encounter such an email.
%\end{recommendation}


%\begin{recommendation}
%Everyone should always double-check the %sender's address for COVID-19 emails to %catch email masquerading.
%\end{recommendation}


%\begin{recommendation}
%Instead of making payments from email links, users should go to the original source website when donating to a COVID-19 cause. 
%\end{recommendation}

\subsubsection{Coordinated cyber security management}
\begin{recommendation}
Security teams should coordinate with decision-makers to setup a compact incident response plans by following standard NIST cybersecurity framework \cite{NIST_framework} against any successful COVID-19 themed attacks. 
\end{recommendation}

\begin{recommendation}
Enterprises should be proactive and adapt to fast changes regarding existing models and frameworks to detect new COVID-19 attacks.
\end{recommendation}


\begin{recommendation}
Maintain cyber hygiene by checking reviews of software before use and discuss new software pros and cons among peers.
\end{recommendation}

%\begin{recommendation}
%Enterprises can encourage their employees to check news and COVID-19 updates only from authorized and reliable sources to avoid misinformation dissemination. They can compile those information sources and share with their employees. 
%\end{recommendation}


%\begin{recommendation}
%Double-checking website addresses may protect individuals either from visiting a typo-squatting and/or visually similar phishing website, or from downloading malware.
%\end{recommendation}


%\begin{recommendation}
%Employees should act responsibly, and they should verify from reliable sources before sharing sensitive news with other colleagues.
%\end{recommendation}


%\begin{recommendation}
%(May not be in scope?) Internet users should not buy or trust testing kits, vaccines, therapies, cures from unreliable sources that are not approved by national or international level health agencies.
%\end{recommendation}



%predicting known attack groups from real-time incident reports and security logs,

%\subsubsection{Awareness safeguards} 
%Moreover, enterprises should actively communicate these risk factors and attack scenarios to train their employees and users. 

%Primarily, All enterprises should communicate their employees on how often and who are going to send emails regarding COVID-19. 
%Suspicious emails may use COVID-19 lures (mentioned in section 3) to emotionally distressed employees with compassionate sentences to become successful. 

%The first wall of defense is the human shield, as most of the attacks need human interaction and error to be victorious. 
%Enterprises should teach their employees on hidden email links and how hovering over a link can discover the real website (or domain address). 

%We should not download untrusted third-party VPN, remote access, and virtual meeting software. 

 
\subsection{Recommendations Against Rising Non-COVID-19 Themed Cyberattacks}
Along with the rise in COVID-19 themed cyber attacks as discussed in section \ref{sec:methodology}, we are also observing other state-of-the-art non-COVID-themed attacks gaining recent interest because of added incentives amid COVID-19 pandemic. We are listing those attacks as we understand being informed and vigilant as a community can help us stay safe. 
\subsubsection{Ransomware attacks}
Ransomware is a special kind of malware and propagates similarly through websites, emails, and mobile applications. Thus, securing this artifacts may also provide proactive security against ransomware attacks as well. However, some advanced multi-stage attacks (APTs) may target healthcare and COVID-19 research facilities with ransomware attacks. Compliance with standard cyber hygiene and best security practices should keep enterprise safe from ransomware attacks \cite{CISA_ransomware, hornetsec_ransomware}. Moreover, enterprise should be vigilant about new zero-day CVEs and software vulnerabilities to keep their enterprise network safe.

\subsubsection{Impersonation attacks}
Since COVID-19 pandemic force us to go virtual for business continuity, it creates opportunity for attackers to impersonate as legitimate entities (e.g., government, doctor, CEO, WHO) and make fraud transactions, compromise business emails, and other similar attacks. Usually, impersonation attacks are carried out through emails, chats, phone calls, and SMSs. As per recommendations \ref{rec:mfa} and \ref{rec:awareOnlure}, enterprises should inform their employees on such lures and enforce MFA for all critical transactions and communications during this pandemic. 

%Enterprises also need to communicate these scenarios well ahead so that their customers and employees are aware and do not fall victim to such social engineering attacks. 
%Moreover, fraud donation websites and payment links in email for COVID-19 donations, claiming to support WHO or similar organizations who are fighting from the frontline can be detected by checking the payment methods. If the donation campaigns did not allow users to pay through credit card or PayPal (and similar) payment system instead asking for bank transfers should is a clear indicator of donation scamming. 

\subsubsection{Defense against router DNS hijacking}
Router DNS hijackings are attacks where attackers get remote access to routers and change DNS settings to land victims into attacker controller websites and launch malware or phishing attacks. We have seen reports on these attacks rising during COVID-19 as with active WFH policies attackers have far more incentive than regular times \cite{oski_malware_attack_covid19}. The most effective defense against router DNS hijacking is to practise recommendation \ref{rec:dnsSettingsPass} \cite{DNS_hijack_protection}. Additionally, defenders can raise alerts if the browser automatically redirects from a reputed website to a non-reputed ones because of change in the DNS settings. 

\subsubsection{Defense against Zoom-bombing attacks}
Zoombombing is when an unauthorized person or stranger joins a Zoom meeting/chat session and cause disorder by saying offensive things and even photobombing the meeting by sharing pornographic and hate images. When using Zoom for online classrooms, meetings or events, the host is advised to making meetings private and require a password or use the waiting room feature to control the admittance of additional people.  The links to a teleconference or classroom should be sent directly to the individual participants and never be publicly available on a social media post.  Turn off the annotation feature and restrict other feature as needed in host controls. Those managing a conference in Zoom should change the screen sharing option to “Host-Only.” Finally, you should always run the latest version of Zoom.

\subsubsection{Defense against HTML/XSS injection attacks}
Website and mobile app injections attacks are handy during a pandemic to propagate various malware. These attacks can be far more impactful when injected into a top legitimate website working for COVID-19 related data and updates with large volume of live users. Hence, such organization and website should regularly scan and check for changes in their website HTML contents, added scripts, hidden divisions, and images. 

\ignore{
{\color{red}\footnote{find an appropriate home for this paragraph. I think we can use this as part of the discussion/conclusion to make a final comment on the issue ...}
%discussion on implementing zero-trust securitymodel
VPN alone would not be enough, and large scale use of VPNs may provide enough incentives to attackers for targeting their attacks for VPN vulnerabilities \cite{CyberHyigene_during_COVID19}. We also find discussion from experts \cite{zero_trust_model_for_COVID_cw, zero_trust_model_for_COVID_dr, zero_trust_model_for_COVID_ng} suggesting more stringent approach to implement zero-trust security models \cite{zero_trust_model_citrix, zero_trust_model_cloudflare, zero_trust_model_cso} for enterprise data and network access. This pandemic should give the enterprise leaders a strong message to strengthen security monitoring, proactive defense, and test security software effectiveness regularly.
}}
%These can be summarized from the various website ...
%\subsection{Recommendations Specific to Incidents}

%\subsubsection{Generic Recommendations When There Is No "Stay at Home" Policy}

%e.g., what if it's political event?

%\subsubsection{Generic Recommendations When There Is  "Stay at Home" Policy}

%e.g., what if it's COVID-XX?


==> related-work.tex <==

%\subsection{Defence against malicious URLs and websites}
%In literature, we find end-to-end frameworks for automated phishing URL detection in real-time \cite{AutomatedPhishingDetection}. However, in our case, we are dealing only with the domain name, and no path information is provided, which is more challenging because of the possibility of increasing false-positive rates. Moreover, their framework has 87\% real-time detection accuracy only for phishing URLs, while results for other attacks leveraging malicious websites are not mentioned with similar approaches. 
\ignore{
%rewrite this section by only considering the prior studies that deal with X-themed attacks, for which there should be very few references. then, compare their perspectives against ours ... no need to say much about comparison at the means level; rather, we stay at the goals-level comparsion

}


